A Formalized Extension of the Substitution Lemma in Coq

The substitution lemma is a renowned theorem within the realm of lambda-calculus theory and concerns the interactional behaviour of the metasubstitution operation. In this work, we augment the lambda-calculus's grammar with an uninterpreted explicit substitution operator, which allows the use of our framework for different calculi with explicit substitutions. Our primary contribution lies in verifying that, despite these modifications, the substitution lemma continues to remain valid. This confirmation was achieved using the Coq proof assistant. Our formalization methodology employs a nominal approach, which provides a direct implementation of the alpha-equivalence concept. The strategy involved in variable renaming within the proofs presents a challenge, specially on ensuring an exploration of the implications of our extension to the grammar of the lambda-calculus.

==> eptcsdata.tex <==
\providecommand{\firstpage}{80}
\providecommand{\publicationstatus}{H. Cheval, L. Leu\c{s}tean, A. Sipo\c{s} (Eds.):\\ 7th Symposium on Working Formal Methods (FROM 2023)\\
EPTCS 389, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.389.7}{10.4204/EPTCS.389.7}}
\pdfoutput=1

